DEVIAS: Learning Disentangled Video Representations of Action and Scene

Video recognition models often learn scene-biased action representation due to the spurious correlation between actions and scenes in the training data. Such models show poor performance when the test data consists of videos with unseen action-scene combinations. Although scene-debiased action recognition models might address the issue, they often overlook valuable scene information in the data. To address this challenge, we propose to learn DisEntangled VIdeo representations of Action and Scene (DEVIAS), for more holistic video understanding. We propose an encoder-decoder architecture to learn disentangled action and scene representations with a single model. The architecture consists of a disentangling encoder (DE), an action mask decoder (AMD), and a prediction head. The key to achieving the disentanglement is employing both DE and AMD during training time. The DE uses the slot attention mechanism to learn disentangled action and scene representations. For further disentanglement, an AMD learns to predict action masks, given an action slot. With the resulting disentangled representations, we can achieve robust performance across diverse scenarios, including both seen and unseen action-scene combinations. We rigorously validate the proposed method on the UCF-101, Kinetics-400, and HVU datasets for the seen, and the SCUBA, HAT, and HVU datasets for unseen action-scene combination scenarios. Furthermore, DEVIAS provides flexibility to adjust the emphasis on action or scene information depending on dataset characteristics for downstream tasks. DEVIAS shows favorable performance in various downstream tasks: Diving48, Something-Something-V2, UCF-101, and ActivityNet. The code is available at https://github.com/KHU-VLL/DEVIAS.

==> 3_overview.tex <==
\section{Preliminaries and Baselines}
\label{sec:overview}
\subsection{Vision Transformer}
% Introduce your problem with a toy example
First, we briefly examine the Vision Transformer model in the context of videos. In all our experiments, we employ the architecture of videoMAE \cite{videomae} as the backbone. We takes RGB videos as inputs, $I \in \mathbb{R}^{B\times 2T\times H\times W\times C}$, consisting of $B$ videos of $2T$ frames, $H \times W$ spatial dimensions, and $C$ channels.
Additionally, we utilize 3D convolution to employ patch embeddings $I$ into $2 \times p \times p$. 
We add a fixed positional embedding \(p_e\) to these patches, resulting in the final input patches, $X \in \mathbb{R}^{B \times TN \times D}$, for the attention blocks \eqref{eq:input}. 
Another commonly employed method involves appending a learnable token \cite{vit} \eqref{eq:cls_input}.


\begin{equation}
\label{eq:input}
    {\mathbf{X_{0}}} = [{\bx}^{1}, {\bx}^{2}, \cdots, {\bx}^{TN}] + \bp_{e}
\end{equation}

\begin{equation}
\label{eq:cls_input}
        {\mathbf{X_{0}}} = [\{\cls\}, {\bx}^{1}, {\bx}^{2}, \cdots, {\bx}^{TN}] + \bp_{e}
\end{equation}

And then, we adopt the Multi-Head Self-Attention block architecture of ViT. We feed input patches \(X\) int \(L\) blocks.
    \begin{equation}
    \begin{aligned}
        \bz_{l} = \bX_{l-1} &+ \mha(\lnorm(\bX_{l-1})),  \\
        \bX_{l} = \bz_{l} &+ \mlp(\lnorm(\bz_{l})),
    \end{aligned}\label{equ:transformer}
    \end{equation}
where LN \cite{layernorm}, MHA \cite{vit}, and MLP refer to layer normalization, multi-head self-attention, and multi-layer perceptron, respectively, with a skip connection added. In ViT, the shape of the input pathes \(X_l\) remains consistent through the \(l\)-th blocks. 



Therefore, the output from the last block of ViT serves as the input to a single FC layer as the classifier.
\begin{equation}
\label{eq:classifier_pooling}
\begin{aligned}
        L(\mathbb{C}(AvgPool[\mathbf{X}]),\mathbf{y}),  \qquad   \mathbb{C} \in\mathbb{R}^{N_a\times D} \\
        L(\mathbb{C}(\cls),\mathbf{y}),  \qquad   \mathbb{C} \in\mathbb{R}^{N_a\times D}
\end{aligned}
    \end{equation}
Given that \(N_a\) represents the number of action labels and \(D\) denotes the embedding dimension of the patch, there are two scenarios. If a learnable cls token is present, it serves as the input to the classifier. In the absence of this cls token, the \(NT\) patches undergo average mean pooling to form the input for the classifier. And typically, training is done using the ground truth \(y\) with a cross-entropy loss.

% This figure illustrate the overall process of the algorithm, starting from inputs, processing steps, and outputs. Use forward references the figures with the corresponding equations and sections in the paper.

\subsection{Baselines}
In our setting, We have video \(v\) with an action label \(y_a\) and pseudo scene label \(y_s\), employing a VIT model trained on Places365 \cite{places365}. Our goal is to train a single model that recognizes both the foreground (action) and background (scene) of a video. To achieve this, the simplest baseline approach introduces two learnable tokens, each guiding the model to learn the action and scene respectively (\texttt{TwoToken}). The model is trained using the following equation:
\begin{equation}
        {\mathbf{X_{0}}} = [\texttt{[CLS$_{action}$,CLS$_{scene}$]}
        , {\bx}^{1}, {\bx}^{2}, \cdots, {\bx}^{TN}] + \bp_{e}
\end{equation}

\begin{equation}
\begin{aligned}    
        L(\mathbb{C}_{\text{a}}(\texttt{[CLS$_{action}$]}),\mathbf{y_a}),  \qquad   \mathbb{C}_{\text{a}} \in\mathbb{R}^{N_a\times D} \\
        L(\mathbb{C}_{\text{s}}(\texttt{[CLS$_{scene}$]}),\mathbf{y_s}),  \qquad   \mathbb{C}_{\text{s}} \in\mathbb{R}^{N_s\times D}
\end{aligned}   
\end{equation}

where \(N_a\) represents the number of action labels and \(N_s\) denotes the number of scene labels. The cls tokens are each fed into their respective heads for training. 

Another baseline employs a unified head (\texttt{TwoToken-Unified}) by the following equation:

\begin{equation}
\begin{aligned}    
        L(\mathbb{C}(\texttt{[CLS$_{action}$]}),\mathbf{y_a}),  \qquad   \mathbb{C} \in\mathbb{R}^{(N_a+N_s)\times D} \\
        L(\mathbb{C}(\texttt{[CLS$_{scene}$]}),\mathbf{y_s}),  \qquad   \mathbb{C} \in\mathbb{R}^{(N_a+N_s)\times D}
\end{aligned}   
\end{equation}

\texttt{TwoToken-Unified} learns using a single integrated head. Utilizing this unified head naturally leads the action cls token to acquire a lower prediction for the scene, hence training to exclude mutual information. Similarly, the scene cls token inherently holds a reduced probability for action.

While the baseline approach is intuitive and seems reasonable, the high correlation between action labels and background labels results in the action and background features being heavily entangled shown in \tabref{knn_reverse} and \figref{umap}

==> figure/fig_attention_umap.tex <==
\begin{figure}[t]
    \mpage{0.23}{
        \centering    
        \includegraphics[width=\linewidth]{figure/img_files/umap1.pdf}
    }    
    \mpage{0.23}{
        \centering
        \includegraphics[width=\linewidth]{figure/img_files/umap2.pdf}
    }    
    \mpage{0.23}{
        \centering
        \includegraphics[width=\linewidth]{figure/img_files/umap_be.pdf}
    }     
    \mpage{0.23}{
        \centering
        \includegraphics[width=\linewidth]{figure/img_files/umap3.pdf}
    }     

    \mpage{0.23}{\fontsize{5.5pt}{10pt}\selectfont (a) Two-Token.}    
    \mpage{0.23}{\fontsize{5.5pt}{10pt}\selectfont (b) Two-Token w/ BE~\cite{BE}.}   
    \mpage{0.23}{\centering \fontsize{5.5pt}{10pt}\selectfont (c) Two-Token w/ FAME~\cite{fame}.} 
    \mpage{0.23}{\fontsize{5.5pt}{10pt}\selectfont (d) DEVIAS.}

    \captionof{figure}{
    \textbf{UMAP~\cite{mcinnes2018umap} visualization on UCF-101, test split.} 
    \red{Red}/\blue{blue} dots are action/scene feature vectors. 
    %
    DEVIAS demonstrates a distinct separation between action and scene feature vectors.
    }
    \figcapmargin    
    \label{fig:umap}

\end{figure}
% \vspace{-0.5em}  %cameraready

% \begin{figure}[t]
% \mpage{0.49}{
%     \mpage{0.06}{\fontsize{5pt}{10pt}\selectfont Input 
%     Frame
%     }    
%     \hfill
%     \mpage{0.39}{
%         \centering
%         \includegraphics[width=\linewidth]{figure/img_files/slot_viz_ucf_1.pdf}
%     }
%     \hfill
%     \mpage{0.39}{
%         \centering
%         \includegraphics[width=\linewidth]{figure/img_files/slot_viz_hat_1.pdf}
%     }
%     \vspace{-1.1em}
    
%     \mpage{0.06}{
%     \fontsize{5pt}{10pt}\selectfont Action
%     Slot
%     } 
%     \hfill
%     \mpage{0.39}{
%         \centering
%         \includegraphics[width=\linewidth]{figure/img_files/slot_viz_ucf_2.pdf}
%     } 
%     \hfill
%     \mpage{0.39}{
%         \centering    
%         \includegraphics[width=\linewidth]{figure/img_files/slot_viz_hat_2.pdf}
%     }
%     \vspace{-1.1em}
    
%     \mpage{0.06}{
%     \fontsize{5pt}{10pt}\selectfont Scene
% Slot
%     }   
%     \hfill
%     \mpage{0.39}{
%         \centering
%         \includegraphics[width=\linewidth]{figure/img_files/slot_viz_ucf_3.pdf}
%     }
%     \hfill
%     \mpage{0.39}{
%         \centering    
%         \includegraphics[width=\linewidth]{figure/img_files/slot_viz_hat_3.pdf}
%     }
%     % \vspace{-1.7em}
%     \vspace{-0.7em}


%     % \mpage{0.06}{}\hfill
%     % \mpage{0.41}{\fontsize{5pt}{10pt}\selectfont (a) Seen combination.}
%     % \hfill
%     % \mpage{0.41}{\fontsize{5pt}{10pt}\selectfont (b) Unseen combination.}
%     \mpage{0.06}{}
%     \hspace{2.1pt}
%     % \hfill
%     \mpage{0.05}{\fontsize{5pt}{10pt}\selectfont (a)}
%     \hspace{1.85cm}
%     \mpage{0.04}{\fontsize{5pt}{10pt}\selectfont (b)}

%     \vspace{-0.5em}

%     \caption{\textbf{Visualization of slot attention map.}
%         (a) Seen combination video from UCF-101~\cite{soomro2012ucf101}, (b) Unseen combination video from HAT Far~\cite{chung2022hatdataset}. Each slot attends to action and scene regions well.
%         % across frames regardless of seen or unseen scenarios.
%         }
%     \figcapmargin
%     \label{fig:attn}
% }    
% \hfill
% \mpage{0.49}{
%     \mpage{0.10}{}
%     % \mpage{0.33}{
%     \mpage{0.3}{
%         \centering    
%         \includegraphics[width=\linewidth]{figure/img_files/umap1.pdf}
%     }    
%     \mpage{0.25}{}
%     \mpage{0.3}{
%         \centering
%         \includegraphics[width=\linewidth]{figure/img_files/umap2.pdf}
%     }    
%     \figcapmargin
%     \\
%     % \hfill    
%     % \mpage{0.25}{}
%     \hspace{0.7cm}
%     \mpage{0.27}{\fontsize{5.5pt}{10pt}\selectfont (a) Two-Token.}    
%     % \hfill
%     \mpage{0.52}{\fontsize{5.5pt}{10pt}\selectfont (b) Two-Token w/ BE~\cite{BE}.}   

%     \\
%     % \vspace{-1em}
    
%     \mpage{0.10}{}
%     \mpage{0.3}{
%         \centering
%         \includegraphics[width=\linewidth]{figure/img_files/umap_be.pdf}
%     }     
%     \mpage{0.25}{}
%     \mpage{0.3}{
%         \centering
%         \includegraphics[width=\linewidth]{figure/img_files/umap3.pdf}
%     }        
%     \figcapmargin

%     \\
%     \hspace{0.002cm}
%     \mpage{0.54}{\centering \fontsize{5.5pt}{10pt}\selectfont (c) Two-Token w/ FAME~\cite{fame}.} 
%     \hspace{-0.3cm}
%     \mpage{0.25}{\fontsize{5.5pt}{10pt}\selectfont (d) DEVIAS.}
%     \hfill
%     \mpage{0.24}{}

%     \vspace{-0.5em}
%     \captionof{figure}{
%     \textbf{UMAP~\cite{mcinnes2018umap} visualization on UCF-101, test split.} 
%     % (a) Two-Token, (b) Two-Token w/ BE, and (c) Two-Token w/ FAME baselines show entangled action and scene feature vectors. In contrast, (d) our DEVIAS demonstrates a distinct separation between action and scene feature vectors. 
%     \red{Red}/\blue{blue} dots are action/scene feature vectors. 
%     % TT stands for the Two-Token baseline.    
%     % All models are trained on the UCF-101 train split. 
%     %
%     DEVIAS demonstrates a distinct separation between action and scene feature vectors.
%     % Best viewed with zoom and color.
%     }
%     \figcapmargin    
%     \label{fig:umap}
% }

% \end{figure}
% % \vspace{-0.5em}  %cameraready

==> figure/fig_motivation.tex <==
% \begin{center}
%     \centering
%     \includegraphics[width=\linewidth]{figure/motivation.png}
% \captionof{figure}{Teaser figure. Main idea of the paper.}
%     \label{fig:teaser}
% \end{center}


==> figure/fig_slot_viz.tex <==
\begin{figure}[t]
    \mpage{0.06}{\fontsize{7pt}{10pt}\selectfont Input 
    Frame
    }    
    \hfill
    \mpage{0.42}{
        \centering
        \includegraphics[width=\linewidth]{figure/img_files/slot_viz_ucf_1.pdf}
    }
    \hfill
    \mpage{0.42}{
        \centering
        \includegraphics[width=\linewidth]{figure/img_files/slot_viz_hat_1.pdf}
    }
    \vspace{-1em}
    
    \mpage{0.06}{
    \fontsize{7pt}{10pt}\selectfont Action
    Slot
    } 
    \hfill
    \mpage{0.42}{
        \centering
        \includegraphics[width=\linewidth]{figure/img_files/slot_viz_ucf_2.pdf}
    } 
    \hfill
    \mpage{0.42}{
        \centering    
        \includegraphics[width=\linewidth]{figure/img_files/slot_viz_hat_2.pdf}
    }
    \vspace{-1em}
    
    \mpage{0.06}{
    \fontsize{7pt}{10pt}\selectfont Scene
    Slot
    }   
    \hfill
    \mpage{0.42}{
        \centering
        \includegraphics[width=\linewidth]{figure/img_files/slot_viz_ucf_3.pdf}
    }
    \hfill
    \mpage{0.42}{
        \centering    
        \includegraphics[width=\linewidth]{figure/img_files/slot_viz_hat_3.pdf}
    }
    \figcapmargin


    \mpage{0.06}{}\hfill
    \mpage{0.42}{\fontsize{7pt}{10pt}\selectfont (a) Seen combination.}
    \hfill
    \mpage{0.42}{\fontsize{7pt}{10pt}\selectfont (b) Unseen combination.}

    \vspace{-0.5em}

    \caption{\textbf{Visualization of DEVIAS slot attention map.}
        (a) Seen combination video from UCF-101~\cite{soomro2012ucf101}, (b) Unseen combinations video from HAT Far~\cite{chung2022hatdataset}. Each slot attends to action and scene regions well across frames regardless of seen or unseen scenarios.}
    \figcapmargin
    \label{fig:attn}
\end{figure}

==> supp_preamble.tex <==
\usepackage{setspace}

\let\titleold\title
\let\instituteold\institute
\let\authorold\author
% \let\authorrunningold\authorrunning

\renewcommand{\title}[1]{\titleold{#1}\newcommand{\thetitle}{#1}}
\renewcommand{\institute}[1]{\instituteold{#1}\newcommand{\theinstitute}{#1}}
\renewcommand{\author}[1]{\authorold{#1}\newcommand{\theauthor}{#1}}
% \renewcommand{\authorrunning}[1]{\authorrunningold{#1}\newcommand{\theauthorrunning}{#1}}


\newcommand\maketitlesupplementary
   {\newpage
   {\centering \doublespacing 
    {\Large \textbf{\thetitle}} \\
    {\large \textbf{Supplementary Material} \\[-0.5ex]
    % {\normalsize ECCV 2024 Submission \#9270} \\
   }
   }
}

\newcommand{\maketitlesupplementaryfull}
   {
    \subtitle{Supplementary Material\vspace{-1em}}
    \titleold{\thetitle}
    \authorold{\theauthor}
    % \authorrunningold{\authorrunning}
    \instituteold{\theinstitute}
    \maketitle
   }

    
    % {\centering
    % \Large
    % \textbf{\thetitle}\\
    % \vspace{0.5em}
    % {\large \textbf{Supplementary Material}} \\
    %     \theinstitute
    % }
   

%   % Replace authors, institute, and running title with review placeholders
%   \let\maketitleold\maketitle
  % \renewcommand{\maketitle}{\author{Anonymous ECCV \eccv@year{} Submission}%
  %                           \titlerunning{ECCV \eccv@year{} Submission \#\eccv@ID}% 
  %                           \authorrunning{ECCV \eccv@year{} Submission \#\eccv@ID}% 
  %                           \institute{Paper ID \#\eccv@ID}%
  %                           \maketitleold}


% \makeatletter
% \ifeccv@review
%   % Display line numbers
%   \AtBeginDocument{%
%     \linenumbers
%     \linenomathpatch{equation}%
%     \linenomathpatchAMS{gather}%
%     \linenomathpatchAMS{multline}%
%     \linenomathpatchAMS{align}%
%     \linenomathpatchAMS{alignat}%
%     \linenomathpatchAMS{flalign}%
%   }

%   % Crop the page for review version
%   \RequirePackage[width=122mm,left=12mm,paperwidth=146mm,height=193mm,top=12mm,paperheight=217mm]{geometry}

%   % Replace authors, institute, and running title with review placeholders
%   \let\maketitleold\maketitle
%   \renewcommand{\maketitle}{\author{Anonymous ECCV \eccv@year{} Submission}%
%                             \titlerunning{ECCV \eccv@year{} Submission \#\eccv@ID}% 
%                             \authorrunning{ECCV \eccv@year{} Submission \#\eccv@ID}% 
%                             \institute{Paper ID \#\eccv@ID}%
%                             \maketitleold}
% \fi

% \makeatother

==> table/bg.tex <==
\begin{table}[t]
\centering
% \caption{\textbf{Results on Kinetics$\rightarrow$BABEL.} We show the mean class accuracy for the Kinetics$\rightarrow$BABEL dataset. To ensure a fair comparison, we also indicate the views ($clips$ $\times$ $frames$) used in each model. All methods in the table employ I3D as the backbone.}
\caption{BG feature test, Kinetics, \bkh{add HAT}}


\resizebox{1\columnwidth}{!}{
%\fontsize{7.5pt}{9.5pt}\selectfont
\begin{tabular}{ l c c c c c cc |c c}
      \toprule
 \multirow{2}{*}{Method} & \multirow{2}{*}{Pretrain}& \multirow{2}{*}{FG signal} & \multirow{2}{*}{BG signal} & \multicolumn{2}{c}{Kinetics400 (↑)} & \multicolumn{2}{c}{BG} & \multirow{2}{*}{Places365 (↑)} & \multirow{2}{*}{Scuba-K400-Places365 (↑)} \\
  &&&  & BG-only(Top1) & BG-only(Top5)  & IID(Top1) & IID(Top5) &\\
\midrule
VIT(Places365) & Places365 &x& o  & TBD  & TBD  \\
VideoMAE(bg train) &k400 &x& o  & 45.55 & 82.59 & 50.67 & 86.51 & TBD  &41.53 \\
\midrule

VideoMAE & K400 & eta ~41h  \\
VideoMAE(Aug)& K400 & o & x & 33.45 & 65.72 & 39.86 & 71.60 \\
VideoMAE(BE)& K400 &  eta ~82h\\
VideoMAE(FAME) & K400 & o & x & 33.43 & 64.94 & 39.51 & 70.29 \\
\midrule
One-token  &k400&o& o  & \\

Two-token  &k400&o& o  & 47.56 & 81.52 & 53.83 & 86.38 & & 51.43  \\
 %BG-only acc : Two-token(FAME)  &VIT&o& o  & 44.98 & 81.49 & TBD & & \\
Two-token(FAME)  &VIT&o& o  & 46.37 & 82.73 & 52.87 & 87.27 & \\
Two-token (Unified) &k400&o & o  & 47.43 & 81.85 & TBD &TBD & TBD  \\

\midrule

Ours &k400 &o& o  & TBD & TBD  & TBD &TBD & TBD\\
\bottomrule
\end{tabular}
}

\label{tab:hat}
\end{table}

\begin{table}[t]
\centering
% \caption{\textbf{Results on Kinetics$\rightarrow$BABEL.} We show the mean class accuracy for the Kinetics$\rightarrow$BABEL dataset. To ensure a fair comparison, we also indicate the views ($clips$ $\times$ $frames$) used in each model. All methods in the table employ I3D as the backbone.}
\caption{BG feature test, UCF}


\resizebox{1\columnwidth}{!}{
%\fontsize{7.5pt}{9.5pt}\selectfont
\begin{tabular}{ l c c c c c c c |c c}
      \toprule
 \multirow{2}{*}{Method} & \multirow{2}{*}{Pretrain}& \multirow{2}{*}{FG signal} & \multirow{2}{*}{BG signal} & \multicolumn{2}{c}{UCF101 (↑)} & \multicolumn{2}{c}{BG} & \multirow{2}{*}{Places365 (↑)} & \multirow{2}{*}{SCUBA(U-P)(↑)} \\
  &&&  & BG-only(Top1)  &BG-only(Top5)& IID(Top1) & IID(Top5) & & \\
\midrule
VIT(Places365) & Places365 &x& o & &  &  \\
VideoMAE(bg train) &UCF101 &x& o  & 30.72 & 61.70 & 43.48 & 71.95 & TBD & 41.53 \\
\midrule

VideoMAE &UCF101 & o & o  & 25.88 & 50.22 & 37.67 & 62.94 & & 8.75 \\
VideoMAE(Aug) &UCF101 & o & o & 27.25 & 52.02 & 38.51 & 64.02 & & 9.76 \\
VideoMAE(BE) &UCF101 & o & o & 26.80 & 51.70 & 38.67 & 63.55 &ucf_scene_lp/9 & 9.36 \\
VideoMAE(FAME) &UCF101 & o & o & 25.61 & 51.15 & 37.17 & 62.70 & & 9.32 \\

\midrule
One-token  &UCF101&o& o  & \\

Two-token  &UCF101&o& o  & 31.40 & 59.58 & 44.83 & 72.27 & & 18.37 \\
 Two-token(BE)  &UCF101&o& o  & 32.96 & 62.33 & 44.99 & 74.23 & & 19.38  \\
 Two-token(FAME)  &UCF101&o& o  & 32.30 & 61.43 & 45.57 & 73.06 & & 24.35 \\
Two-token (Unified) &UCF101&o & o & 32.36 & 60.96 & 45.31 & 73.17 \\

\midrule

Ours &UCF101 &o& o  & 31.75 & 60.16  & 44.62 & 73.28 & & 20.86 \\
\bottomrule
\end{tabular}
}

\label{tab:hat}
\end{table}


==> table/eccv_rebuttal/cnn.tex <==
\begin{table}[h]
  \centering
  \caption{\textbf{Results with I3D (CNN) backbone.}}
        \centering
        \resizebox{\linewidth}{!}{
        \begin{tabular}{lccccc}
            \toprule   
            \multirow{2}{*}{Method} &  \multicolumn{2}{c}{UCF Action($\uparrow$)} & \multicolumn{2}{c}{UCF Scene($\uparrow$)} & \multirow{2}{*}{H.M.}\\
         \cmidrule(lr){2-3} \cmidrule(lr){4-5} 
        & Seen & Unseen & Seen & Unseen \\
        \cmidrule{1-6}
        Naive Action I3D & 92.0 & 20.7 & - & - & \cellcolor{gray!30}- \\
        Naive Scene I3D & - & - & 77.1 & 68.5 & \cellcolor{gray!30}- \\
        \cmidrule{1-6}
        % Multi-Task I3D & 89.7 & 8.6 & 73.5 & 65.3 & \cellcolor{gray!30}25.6 \\
        Multi-Task I3D & 90.8 & 20.1 & 72.8 & 56.4 & \cellcolor{gray!30}43.4 \\
        Multi-Task I3D w/ FAME & 90.2 & 18.6 & 72.8 & 64.1 & \cellcolor{gray!30}42.5 \\
        \cmidrule{1-6}
        DEVIAS I3D & 91.9 & 29.8 & 76.0 & 67.6 & \cellcolor{gray!30}\textbf{55.3}\\
       \bottomrule
       %  \begin{tabular}{clccccc}
       %      \toprule   
       %      \multirow{2}{*}{Traning Strategy} & \multirow{2}{*}{Method} &  \multicolumn{2}{c}{UCF Action($\uparrow$)} & \multicolumn{2}{c}{UCF Scene($\uparrow$)} & \multirow{2}{*}{H.M.}\\
       %   \cmidrule(lr){3-4} \cmidrule(lr){5-6} 
       %  && Seen & Unseen & Seen & Unseen \\
       %  \cmidrule{1-7}
       %  \multirow{2}{*}{Single-Task} & Naive Action I3D & 92.0 & 20.7 & - & - & - \\
       %  & Naive Scene I3D & - & - & 77.1 & 15.6 & - \\
       %  \cmidrule{1-7}
       %  \multirow{2}{*}{Multi-Task} & Multi-Task & 89.7 & 8.6 & 73.5 & 11.0 \\
       %  % & Two-Token & 90.8 & & 72.8 & \\
       %  \cmidrule{1-7}
       %  Disentangle & DEVIAS (I3D) & 89.7 & & 73.0 & \\
       % \bottomrule
        \end{tabular}
        }
\label{tab:cnn}
\end{table}

% \tabcapmargin
% \vspace{0em}

==> table/eccv_rebuttal/matching_algo.tex <==
\begin{table}[h]
\centering
    \caption{\textbf{Ablation study on matching algorithms.}}
\resizebox{0.9\linewidth}{!}{

    \begin{tabular}{lccccc}
        \toprule
        \multirow{2}{*}{Method} & \multicolumn{2}{c}{UCF Action($\uparrow$)}  & \multicolumn{2}{c}{UCF Scene($\uparrow$)} & \multirow{2}{*}{H.M.}  \\
    \cmidrule(lr){2-3} \cmidrule(lr){4-5} 
        
        & Seen & Unseen & Seen & \multicolumn{1}{c}{Unseen}\\
        \midrule    
        Hard assign & 89.4 & 35.1 & 71.1 & 58.3 & \cellcolor{gray!30}56.4  \\
        Greedy & 87.2 & 37.1 & 69.7 & 56.7 & \cellcolor{gray!30}56.8 \\
        Hungarian & 90.1 & 40.1 & 74.0 & 61.0 & \cellcolor{gray!30}\textbf{60.7}\\
        
        \bottomrule
    \end{tabular}
    }
\label{tab:matching_algo}
\end{table}

\vspace{-1em}
 % \tabcapmargin

==> table/eccv_rebuttal/omnivore.tex <==
\begin{table}[h]
  \centering
  \caption{\textbf{Results with Omnivore pre-trained weights.}}
        \centering
        \resizebox{\linewidth}{!}{
        \begin{tabular}{lccccc}
        \toprule   
        \multirow{2}{*}{Method} &  \multicolumn{2}{c}{UCF Action($\uparrow$)} & \multicolumn{2}{c}{UCF Scene($\uparrow$)} & \multirow{2}{*}{H.M.}\\
         \cmidrule(lr){2-3} \cmidrule(lr){4-5} 
        & Seen & Unseen & Seen & Unseen \\
        \cmidrule{1-6}
        Naive Action Omnivore & 94.1 & 44.0 & - & - & \cellcolor{gray!30}- \\
        Naive Scene Omnivore & - & - & 74.4 & 61.4 & \cellcolor{gray!30}- \\
        \cmidrule{1-6}
        Multi-Task Omnivore & 86.7 & 30.0 & 71.2 & 63.5 & \cellcolor{gray!30}53.6 \\
        Multi-Task Omnivore w/ FAME & 88.8 & 40.1 & 67.1 & 57.1 & \cellcolor{gray!30}58.3 \\
        \cmidrule{1-6}
        % DEVIAS(4) & 97.7 & 73.0 & 69.0 & 62.2 \\
        DEVIAS Omnivore & 98.6 & 65.3 & 80.5 & 73.0 & \cellcolor{gray!30}\textbf{77.6}\\
       \bottomrule
        \end{tabular}
       %  \begin{tabular}{clccccc}
       %      \toprule   
       %      \multirow{2}{*}{Traning Strategy} & \multirow{2}{*}{Method} &  \multicolumn{2}{c}{UCF Action($\uparrow$)} & \multicolumn{2}{c}{UCF Scene($\uparrow$)} & \multirow{2}{*}{H.M.}\\
       %   \cmidrule(lr){3-4} \cmidrule(lr){5-6} 
       %  && Seen & Unseen & Seen & Unseen \\
       %  \cmidrule{1-7}
       %  \multirow{2}{*}{Single-Task} & Naive Action Omnivore & 90.9 & & - & - & - \\
       %  & Naive Scene Omnivore & - & - & 74.4 & & - \\
       %  \cmidrule{1-7}
       %  \multirow{1}{*}{Multi-Task} & Omnivore & 83.4 && & \\
       %  \cmidrule{1-7}
       %  Disentangle & DEVIAS &logs/omnivore/4 && & \\
       % \bottomrule
       %  \end{tabular}
        }
\label{tab:omnivore}
\end{table}
% \vspace{0em}
% \tabcapmargin


==> table/fg_hat.tex <==
\begin{table}[t]
\centering
% \caption{\textbf{Results on Kinetics$\rightarrow$BABEL.} We show the mean class accuracy for the Kinetics$\rightarrow$BABEL dataset. To ensure a fair comparison, we also indicate the views ($clips$ $\times$ $frames$) used in each model. All methods in the table employ I3D as the backbone.}
\caption{HAT, FG feature test (action label)}



\resizebox{1\columnwidth}{!}{
%\fontsize{7.5pt}{9.5pt}\selectfont
\begin{tabular}{ l c c c c ccc c }
      \toprule
 \multirow{2}{*}{Method} &\multirow{2}{*}{Backbone}&  \multirow{2}{*}{FG signal} &\multirow{2}{*}{BG signal} & Kinetics400 (↑)& \multicolumn{3}{c}{Kinetics400-HAT (↑)}  &   \multirow{2}{*}{IID} \\
  &&&  & FG-only  &  Random & Close & Far &   \\
\midrule
% TSN & Res50 &o& x  &TBD  &TBD &&& \\
      
Timesformer & TimeSformer &o& x  &TBD  &TBD &&&  \\
VideoMAE & VIT &o& x  & TBD  & 15.1 & & 12.0 & 76.8 \\
VideoMAE (Aug) & VIT&o & x  & TBD  & 16.7 & 25.7 & 13.1 & 77.6 \\
VideoMAE (BE)  & VIT&o& x & TBD & & 24.9 & 12.6 & 77.6 \\
VideoMAE (FAME)  & VIT&o& x & TBD & 20.7 & 28.6 & 17.3 & 77.8 \\
\midrule

Two-token  &VIT&o& o  & TBD & & & & 75.1 \\
+ FAME & VIT &o& o  & TBD & & & & 75.0 \\

% Two-token (Unfified) & VIT &o& o  & TBD &TBD  &&&\\
\midrule

Ours&VIT  &o& o  & TBD  & 19.6 & 28.4 & 16.2 & \\
\bottomrule
\bigskip
\end{tabular}

}


\label{tab:hat}
\end{table}



==> table/fg_scuba.tex <==


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{table*}[t]
% \centering
% % \caption{\textbf{Results on Kinetics$\rightarrow$BABEL.} We show the mean class accuracy for the Kinetics$\rightarrow$BABEL dataset. To ensure a fair comparison, we also indicate the views ($clips$ $\times$ $frames$) used in each model. All methods in the table employ I3D as the backbone.}
% \def\arraystretch{1.2}
% {\tiny

% %\fontsize{7.5pt}{9.5pt}\selectfont
% \setlength{\tabcolsep}{5.5pt}
% \begin{tabular}{ c| c| c| c | c c c c | c|  c c c|| c }
% \toprule


% \multirow{3}{*}{\shortstack{Learning\\ Signal}} & \multirow{3}{*}{\shortstack{Training \\ Strategy}} &  \multirow{3}{*}{Method} & \multicolumn{5}{c|}{Foreground} & \multicolumn{4}{c||}{Background} & \multirow{3}{*}{H.M.}\\
% \cline{4-12}
% & &  & \multirow{2}{*}{K400} & \multicolumn{4}{c|}{SCUBA-Kinetics400} & \multirow{2}{*}{K400} & \multicolumn{3}{c||}{SCUBA-Kinetics400} &  \\
% \cline{5-8}
% \cline{10-12}
% & & &  & Places365 & VQGAN-CLIP  & \multicolumn{1}{c|}{Sinusoid} & Mean &  & Places365 & \multicolumn{1}{c|}{Inpainted-BG} & Mean &\\
% \hline
      
% \multirow{4}{*}{FG} & \multirow{2}{*}{Conventional} &  w/o Aug  & 76.75& 42.31 &  43.50 &  \multicolumn{1}{c|}{49.91} &45.24 &  & & \multicolumn{1}{c|}{} & & done\\
% & & \shortstack{CutMix, MixUp} & 80.00& 50.68 &  49.41  &  \multicolumn{1}{c|}{57.26} &52.45 & 71.60 & 40.59 & \multicolumn{1}{c|}{65.72} & 53.16& 52.80\\
% \cline{2-12}
% & \multirow{2}{*}{\shortstack{Background \\ Debias}} & BE & & eta 50h? &   & \multicolumn{1}{c|}{} & & & & \multicolumn{1}{c|}{} & & \\
%  & & FAME & 77.78 & 50.00  & 50.77  &  \multicolumn{1}{c|}{56.98} & 52.58 & 70.29 & 36.79 & \multicolumn{1}{c|}{64.94} & 50.87 & 51.57\\
% \cline{1-12}
% \multirow{5}{*}{\shortstack{FG \\+\\BG}} & Multi-Task &  One-Token & &   &    & \multicolumn{1}{c|}{} & & & & \multicolumn{1}{c|}{} & & ing\\
% \cline{2-12}
%  &  \multirow{4}{*}{Disentangle} & Two-Token & 75.11 &  37.09 & 36.36  & \multicolumn{1}{c|}{47.17} & 40.21 & 86.38 & 75.80 & \multicolumn{1}{c|}{81.52} & 78.66 & 53.21 \\
%  & & Two-Token w/ BE & & eta 50h  &    & \multicolumn{1}{c|}{} & & & & \multicolumn{1}{c|}{} & & \\
%  & & Two-Token w/ FAME & 74.98 &  35.75 & 37.55 & \multicolumn{1}{c|}{52.09} & 41.80 & 87.27 & 77.44 & \multicolumn{1}{c|}{82.73} & 80.09& 54.93\\
% \cline{3-13}
%  & & Ours & &  53.11 & 53.96 & \multicolumn{1}{c|}{58.19} & 55.09 & & 66.59 & 77.08 & \multicolumn{1}{c|}{71.86} & \textbf{62.37}\\
 


% \bottomrule

% \end{tabular}
% }
% \caption{SCUBA, kinetics400}

% \label{tab:scuba}
% \end{table*}









% \begin{table*}[t]
% \centering
% \caption{\textbf{Action and scene recognition performance on the Kinetics400 dataset}. We report the Top-1 action recognition accuracy and the Top-5 scene recognition accuracy. We evaluate both in-context and out-of-context recognition performances. We also report the harmonic mean (H.M.) of the action recognition and scene recognition. The  \best{best} and the  \second{second-best} H.M. numbers are highlighted.}

% \def\arraystretch{1.2}

% %\fontsize{7.5pt}{9.5pt}\selectfont
% \resizebox{1.0\linewidth}{!}{
% \begin{tabular}{ l l l c  c c c c  cc  c c  c c }
% \toprule

% \multirow{3}{*}{\shortstack{Supervision}} & \multirow{3}{*}{\shortstack{Training \\ Strategy}} &  \multirow{3}{*}{Method} & \multicolumn{5}{c}{Action($\uparrow$) } & \multicolumn{5}{c}{Scene($\uparrow$)} & \cellcolor{gray!30}\\
% \cline{4-8}
% \cline{10-13}
% & &  & In-Context & \multicolumn{4}{c}{SCUBA-Kinetics400} && In-Context & \multicolumn{1}{c}{Kinetics400} & SCUBA-Kinetics400  &  &  \cellcolor{gray!30}H.M.\\
% \cline{5-8} \cline{11-13}
% & & & Kinetics400 & Places365 & VQGAN-CLIP  & \multicolumn{1}{c}{Sinusoid} & \cellcolor{gray!30}Mean && Kinetics400 &Scene-Only& \multicolumn{1}{c}{Places365}  & \cellcolor{gray!30}Mean & \cellcolor{gray!30}\\

% \midrule
      
% \multirow{4}{*}{Action} & \multirow{2}{*}{Naive} &  Baseline ViT  &  76.8 & 42.3 &  43.5 &  \multicolumn{1}{c}{49.9} &\cellcolor{gray!30}45.24 &&   &   &  \multicolumn{1}{c}{ } & \cellcolor{gray!30} & \cellcolor{gray!30} \\
% & & \shortstack{Baseline ViT w. Aug.} & 77.6 & 50.7&  49.4    &\multicolumn{1}{c}{57.3}   &\cellcolor{gray!30}52.5 && 71.6 & 40.6 &\multicolumn{1}{c}{65.7} & \cellcolor{gray!30}53.2& \cellcolor{gray!30}52.8\\
% \cmidrule{2-14}
% % \midrule
% & \multirow{2}{*}{\shortstack{Scene Debiasing}} & BE \cite{BE}  &   &    &    & \multicolumn{1}{c}{ } &\cellcolor{gray!30}  &&    & &  &\cellcolor{gray!30} &  \cellcolor{gray!30}\\
%  & & FAME \cite{fame} & 77.8 & 50.0  & 50.8  &  \multicolumn{1}{c}{57.0}  &\cellcolor{gray!30}52.6 && 70.3 & 36.8 &\multicolumn{1}{c}{64.9} &\cellcolor{gray!30}50.9 & \cellcolor{gray!30}51.6\\
% % \cline{1-14}

% \midrule

% Scene & Naive & Baseline ViT & - & - & - & \multicolumn{1}{c}{-} & \cellcolor{gray!30}- && TODO &  & \multicolumn{1}{c}{} & \cellcolor{gray!30} & \cellcolor{gray!30}- \\

% \midrule

%  & Multi-Task &  One-Token & & TODO & & \multicolumn{1}{c}{} & \cellcolor{gray!30} & &  & \multicolumn{1}{c}{} &  & \cellcolor{gray!30} & \cellcolor{gray!30} \\
% \cmidrule{2-14}
% % \midrule
% Action &  \multirow{4}{*}{Disentangle} & Two-Token & 75.1& 37.1   & 36.4     & \multicolumn{1}{c}{47.2} &\cellcolor{gray!30}40.2 && 86.4 & 75.8 & \multicolumn{1}{c}{81.5} &\cellcolor{gray!30}78.7&  \cellcolor{gray!30}53.2\\
%   \& & & Two-Token w. BE \cite{BE} & TODO & & & & \cellcolor{gray!30} & & & & &\cellcolor{gray!30} &\cellcolor{gray!30}\\
% Scene & & Two-Token w. FAME \cite{fame} & 75.0 & 35.8  & 37.6    &\multicolumn{1}{c}{52.1} &\cellcolor{gray!30}41.8  && 87.3 & 77.4 &\multicolumn{1}{c}{82.7} & \cellcolor{gray!30}80.1& \cellcolor{gray!30}\second{54.9}\\
% % \cline{3-13}
%  & & DEVIAS & TODO & 53.1   & 54.0    &  \multicolumn{1}{c}{58.2} &\cellcolor{gray!30}55.1 &&     &  66.6 & \multicolumn{1}{c}{77.1} &\cellcolor{gray!30}71.9 & \cellcolor{gray!30}\best{62.4}\\
%  % \midrule
% % \midrule
% % Scene & Naive & Baseline ViT & - & - & - & \multicolumn{1}{c}{-} & \cellcolor{gray!30}- && 72.0 & 61.7 & \multicolumn{1}{c}{41.5} & \cellcolor{gray!30}51.6 & \cellcolor{gray!30}- \\

% \bottomrule
% \end{tabular}







% }
% \label{tab:scuba}
% \end{table*}

























%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{table}[t]
\caption{SCUBA, kinetics400}
\resizebox{1\columnwidth}{!}{
%\fontsize{7.5pt}{9.5pt}\selectfont
\begin{tabular}{ l| c| c c  c  cc | c cc }
      \toprule
 \multirow{2}{*}{Train} & \multirow{2}{*}{Method} &\multicolumn{3}{c}{Kinetics400-SCUBA (↑)} &  \multirow{2}{*}{IID} & \multicolumn{3}{c}{\multirow{2}{*}{GAP} }\\
  && Place365 & VQGAN-CLIP  & Sinusoid & &\\
\midrule
      
VideoMAE  & \multirow{4}{*}{x} & 42.31 &  43.50  & 49.91 & 76.75& done\\
VideoMAE (Aug)&  & 50.68  & 49.41  &57.26& 77.6 & ref\\
VideoMAE (BE) & &  - & - & - & - & \\
VideoMAE (FAME) & &  50.00 & 50.77  & 56.98 & 77.78 &\\
%25.74
\midrule

Two-token & \multirow{3}{*}{o}& 37.09  & 36.36 & 47.17 & 75.11 &\\
Two-token (FAME) &  & 44.22  & 46.83 & 52.09 & 74.98 &ing\\
Two-token (BE) &  & - & - & - & - \\
Two-token (Unfified)&  & 35.75  & 37.55 & 46.38 & &ing\\
\midrule

Ours&o  & 58.17  & TBD  &TBD & &\\
\bottomrule
\bigskip
\end{tabular}
\vspace{10pt}
}

\label{tab:scuba_k400}
\end{table}








\begin{table}[t]
\centering
\caption{SCUBA, UCF101}

\resizebox{1\columnwidth}{!}{
%\fontsize{7.5pt}{9.5pt}\selectfont
\begin{tabular}{ l c c c c c | c cc }
      \toprule
 \multirow{2}{*}{Method} &  \multirow{2}{*}{bg signal}&\multicolumn{3}{c}{UCF101-SCUBA (↑)} &    FG & \multicolumn{3}{c}{\multirow{2}{*}{GAP} }\\
  && Place365 & VQGAN-CLIP  & Sinusoid & IID \\
\midrule
      
VideoMAE  & \multirow{4}{*}{x} & 15.01 & 12.35  & 20.95  & 92.92 & done\\
VideoMAE (Aug)&  &  19.10 &18.77 &19.38 & 91.30 & ref\\
VideoMAE (BE) & &  16.11 & 12.13 & 38.66  & 92.33 & logs/ucf_slot/68\\
VideoMAE (FAME) & &  22.00 & 24.75 & 15.63 & 91.62 &\\
\midrule
One-token & \\
Two-token & \multirow{3}{*}{o}&  11.87 &  11.05 & 19.85 & 85.96 &\\
Two-token (FAME) &  & 21.65  & 25.27 & 15.27  & 89.51 &ing\\
Two-token (BE)&  & 14.99 & 13.08 & 20.51 & 89.93 \\

Two-token (Unfified)&  & 13.54 &  11.67 & 20.86 & 86.28 &ing\\
\midrule

Ours&  o & \textbf{41.03}  & 41.83  & 40.62 & 90.11&\\
\bottomrule
\vspace{10pt}
\bigskip
\end{tabular}
}


% HMDB MAE pretrain and HMDB train pretrain chekpoint not available
% \resizebox{1\columnwidth}{!}{
% %\fontsize{7.5pt}{9.5pt}\selectfont
% \begin{tabular}{ l c c c c    c| c cc }
%       \toprule
%  \multirow{2}{*}{Method} &  \multirow{2}{*}{bg signal}&\multicolumn{3}{c}{HMDB-SCUBA (↑)} &    \multirow{2}{*}{HMDB51} & \multicolumn{3}{c}{\multirow{2}{*}{GAP} }\\
%   && Place365 & VQGAN-CLIP  & Sinusoid & &\\
% \midrule
      
% VideoMAE  & \multirow{4}{*}{x} &  & TBD  &TBD  & & done\\
% VideoMAE (Aug)&  &  23.24& 27.19& 18.55 &62.60  & ref\\
% VideoMAE (BE) & &  TBD &TBD   &TBD  && ing\\
% VideoMAE (FAME) & &  TBD &TBD   &TBD  &&\\
% \midrule

% Two-token & \multirow{3}{*}{o}&  &  &TBD & &\\
% Two-token (FAME) &  & TBD  & TBD &TBD & &ing\\

% Two-token (Unfified)&  &  &  &TBD & &ing\\
% \midrule

% Ours&o  & TBD  & TBD  &TBD & &\\
% \bottomrule
% \bigskip
% \end{tabular}
% }

\label{tab:scuba_ucf}
\end{table}


==> table/fusion_test.tex <==

\begin{table}[t]
\centering

\caption{downstream fusion linear probe}

% \resizebox{0.9\columnwidth}{!}{
\fontsize{7.5pt}{9.5pt}\selectfont
\begin{tabular}{ l c c c}
      \toprule
Method  &  UCF-101 & UCF-101 (scene biased) & Diving48 \\
\midrule
Action Baseline ViT & 97.1 &&21.0 \\
Action Baseline ViT w. Aug. &97.0&  &19.6 \\
BE \cite{fame} &97.7 & & 23.35 \\
FAME \cite{fame} &97.4 & &  21.3\\
Scene Baseline ViT  &\\
\midrule
Action slot only & & \\
Scene slot only & & \\
slots concat   &97.5& & 21.47\\
slots concat (mlp)   &97.57& & \\
slots sum  & 97.4 && 21.12\\
\bottomrule
\end{tabular}
\label{tab:fusion}
\end{table}

\begin{table}[t]
\centering

\caption{downstream fusion linear probe ucf pretrained}

% \resizebox{0.9\columnwidth}{!}{
\fontsize{7.5pt}{9.5pt}\selectfont
\begin{tabular}{ l c c c}
      \toprule
Method  &  HMDB51 &\\
\midrule
Action Baseline ViT & 59\\
BE & 64\\
\midrule
fg-only & \\
bg-only & \\
slot concat & 50\\
slot sum & 50\\

\bottomrule
\end{tabular}
\label{tab:fusion}
\end{table}


% \begin{table}[t]
% \centering

% \caption{downstream fusion linear probe ucf pretrained}

% % \resizebox{0.9\columnwidth}{!}{
% \fontsize{7.5pt}{9.5pt}\selectfont
% \begin{tabular}{ l c c c}
%       \toprule
% Method  &  HAT-Far &\\
% \midrule
% Action Baseline ViT & 22.7 \\
% FAME & 27.98 \\
% \midrule
% fg-only & \\
% bg-only & \\
% slot concat & 5.48 \\
% slot sum & 6.13 \\

% \bottomrule
% \end{tabular}
% \label{tab:fusion}
% \end{table}

\begin{table}[t]
\centering
\caption{downstream fusion linear probe kinetics pretrained}

% \resizebox{0.9\columnwidth}{!}{
\fontsize{7.5pt}{9.5pt}\selectfont
\begin{tabular}{ l c c c}
      \toprule
Method  &  HAT-Far &\\
\midrule
Action Baseline ViT & 22.1 \\
FAME &  \\
\midrule
fg-only & 25.9 \\
bg-only & \\
slot concat &  \\
slot sum &  \\

\bottomrule
\end{tabular}
\label{tab:fusion}
\end{table}

==> table/kinetics400_extra.tex <==
% total ver
\begin{table*}[t]
\centering
\caption{\textbf{Action and scene recognition performance on the Kinetics-400 dataset}. We report the Top-1 action recognition accuracy and the Top-5 scene recognition accuracy. We evaluate both in-context and out-of-context recognition performances. We also report the harmonic mean (H.M.) of the action recognition and scene recognition. The  \best{best} and the  \second{second-best} H.M. numbers are highlighted. $\dagger$ indicates that we are evaluating the performance under contrasting supervision, for which we employ a linear probe approach.}

\def\arraystretch{1.2}

%\fontsize{7.5pt}{9.5pt}\selectfont
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{ lll c ccc ccc c  c  c c ccc c c c }
\toprule

\multirow{3}{*}{\shortstack{Supervision}} & \multirow{3}{*}{\shortstack{Training \\ Strategy}} &  \multirow{3}{*}{Method} & \multicolumn{8}{c}{Action($\uparrow$) } & \multicolumn{7}{c}{Scene($\uparrow$)} & \cellcolor{gray!30}w/o iid & \cellcolor{gray!30} w/ iid\\
\cline{4-11}
\cline{13-18}
& &  & In-Context & \multicolumn{3}{c}{SCUBA-Kinetics-400} & \multicolumn{3}{c}{HAT-Kinetics-400} &&& In-Context & \multicolumn{1}{c}{Kinetics-400} & \multicolumn{3}{c}{HAT-Kinetics-400}  &  &  \cellcolor{gray!30}H.M. & \cellcolor{gray!30}H.M.\\
\cline{5-11} \cline{14-18}
& & & Kinetics-400 & Places365 & VQGAN-CLIP  & Sinusoid & Random & Close & \multicolumn{1}{c}{Far} & \cellcolor{gray!30}Mean && Kinetics-400 &Scene-Only& Random & Close & Far & \cellcolor{gray!30}Mean & \cellcolor{gray!30} &  \cellcolor{gray!30}\\

\midrule
      
\multirow{4}{*}{Action$\dagger$} & \multirow{2}{*}{Naive} &  Baseline ViT  &  76.8 & 42.3 &  43.5 & 49.9 & 15.1 & 23.9 & 12.0 &\cellcolor{gray!30}31.1&&   71.2&   65.8&  \multicolumn{1}{c}{63.3} & 64.8& 65.7 & \cellcolor{gray!30}64.9& \cellcolor{gray!30}42.1& \cellcolor{gray!30}48.0 \\
& & \shortstack{Baseline ViT w/ Aug.} & 77.6 & 50.7&  49.4    &\multicolumn{1}{c}{57.3} & 16.7 & 25.7 & 13.1  &\cellcolor{gray!30}35.5&& 71.6 & 65.7 &\multicolumn{1}{c}{63.9} & 66.4& 65.7 &  \cellcolor{gray!30}65.4& \cellcolor{gray!30}46.0& \cellcolor{gray!30}51.2\\
\cmidrule{2-20}
% \midrule
& \multirow{2}{*}{\shortstack{Scene Debiasing}} & BE \cite{BE}  &   77.6&    44.3&    44.3& \multicolumn{1}{c}{52.0} & 15.7 & 24.9 & 12.6 &\cellcolor{gray!30}32.3& & 70.7 & 65.4 & 63.7 & 66.3& 65.7 &\cellcolor{gray!30}65.3&  \cellcolor{gray!30}43.2& \cellcolor{gray!30}48.9 \\
 & & FAME \cite{fame} & 77.8 & 50.0  & 50.8  &  \multicolumn{1}{c}{57.0} & 20.7 & 28.6 & 17.3 &\cellcolor{gray!30}37.4&& 70.3 & 64.9 &\multicolumn{1}{c}{61.7} & 64.4&  64.5 &\cellcolor{gray!30}63.9& \cellcolor{gray!30}\second{47.2}& \cellcolor{gray!30}\second{51.9}\\
% \cline{1-14}

\midrule

Scene$\dagger$ & Naive & Baseline ViT & 43.0 & 9.8 & 8.0 & \multicolumn{1}{c}{15.8} & 3.0 & 9.5 & 1.9 & \cellcolor{gray!30}8.0&& 86.5&  82.6& \multicolumn{1}{c}{81.2} & 82.4& 81.7 & \cellcolor{gray!30}82.0& \cellcolor{gray!30}14.6 & \cellcolor{gray!30}22.5\\

\midrule

 & Multi-Task &  One-Token & 74.2 & 35.3 & 36.4 & \multicolumn{1}{c}{46.2} & 12.2 & 21.8 & 9.1 & \cellcolor{gray!30}26.8& & 87.9 & \multicolumn{1}{c}{83.8} & 82.6 & 83.4& 83.3 & \cellcolor{gray!30}83.3 & \cellcolor{gray!30}40.6 & \cellcolor{gray!30}48.0\\
\cmidrule{2-20}
% \midrule
Action &  \multirow{4}{*}{Disentangle} & Two-Token & 75.1& 37.1   & 36.4     & \multicolumn{1}{c}{47.2} & 13.1 & 21.8 & 10.0 &\cellcolor{gray!30}27.6&& 86.4 & 75.8 & \multicolumn{1}{c}{80.1} & 81.9& 81.4 &\cellcolor{gray!30}79.8&  \cellcolor{gray!30}41.0& \cellcolor{gray!30}48.3\\
  \& & & Two-Token w/ BE \cite{BE} & 75.1 & 37.4 & 37.3 & 48.0& 13.6 & 22.7 & 10.3 & \cellcolor{gray!30}28.2& & 87.7 & 82.9 & 81.4 & 82.9& 83.1 &\cellcolor{gray!30}82.6 &\cellcolor{gray!30}42.1 & \cellcolor{gray!30}49.3\\
Scene & & Two-Token w/ FAME \cite{fame} & 75.0 & 35.8  & 37.6    &\multicolumn{1}{c}{52.1} & 18.1 & 25.9 & 14.9 & \cellcolor{gray!30}30.7&& 87.3 & 77.4 &\multicolumn{1}{c}{81.9} & 84.1& 84.0 & \cellcolor{gray!30}81.9& \cellcolor{gray!30}44.7& \cellcolor{gray!30}51.2\\
% \cline{3-13}
 & & DEVIAS & 77.3 & 51.8& 53.0&  \multicolumn{1}{c}{59.7} & 20.1 & 28.6 & 16.9 &\cellcolor{gray!30}38.4&& 82.0 &  76.5& \multicolumn{1}{c}{75.8} & 78.6& 78.0 &\cellcolor{gray!30}77.2& \cellcolor{gray!30}\best{51.2}& \cellcolor{gray!30}\best{56.2}\\
 % \midrule
% \midrule
% Scene & Naive & Baseline ViT & - & - & - & \multicolumn{1}{c}{-} & \cellcolor{gray!30}- && 72.0 & 61.7 & \multicolumn{1}{c}{41.5} & \cellcolor{gray!30}51.6 & \cellcolor{gray!30}- \\

\bottomrule
\end{tabular}

}
\label{tab:scuba}
\end{table*}




% with SCUBA-bg
% \begin{table*}[t]
% \centering
% \caption{\textbf{Action and scene recognition performance on the Kinetics-400 dataset}. We report the Top-1 action recognition accuracy and the Top-5 scene recognition accuracy. We evaluate both in-context and out-of-context recognition performances. We also report the harmonic mean (H.M.) of the action recognition and scene recognition. The  \best{best} and the  \second{second-best} H.M. numbers are highlighted. $\dagger$ indicates evaluating the performance of contrasting supervision, we adapt linear probe.}

% \def\arraystretch{1.2}

% %\fontsize{7.5pt}{9.5pt}\selectfont
% \resizebox{1.0\linewidth}{!}{
% \begin{tabular}{ l l l c  c c c c  cc  c c  c c }
% \toprule

% \multirow{3}{*}{\shortstack{Supervision}} & \multirow{3}{*}{\shortstack{Training \\ Strategy}} &  \multirow{3}{*}{Method} & \multicolumn{5}{c}{Action($\uparrow$) } & \multicolumn{5}{c}{Scene($\uparrow$)} & \cellcolor{gray!30}\\
% \cline{4-8}
% \cline{10-13}
% & &  & In-Context & \multicolumn{4}{c}{SCUBA-Kinetics-400} && In-Context & \multicolumn{1}{c}{Kinetics-400} & SCUBA-Kinetics-400  &  &  \cellcolor{gray!30}H.M.\\
% \cline{5-8} \cline{11-13}
% & & & Kinetics-400 & Places365 & VQGAN-CLIP  & \multicolumn{1}{c}{Sinusoid} & \cellcolor{gray!30}Mean && Kinetics-400 &Scene-Only& \multicolumn{1}{c}{Places365}  & \cellcolor{gray!30}Mean & \cellcolor{gray!30}\\

% \midrule
      
% \multirow{4}{*}{Action$\dagger$} & \multirow{2}{*}{Naive} &  Baseline ViT  &  76.8 & 42.3 &  43.5 &  \multicolumn{1}{c}{49.9} &\cellcolor{gray!30}45.2 &&   71.2&   65.8&  \multicolumn{1}{c}{40.8} & \cellcolor{gray!30}53.3 & \cellcolor{gray!30}48.9 \\
% & & \shortstack{Baseline ViT w/ Aug.} & 77.6 & 50.7&  49.4    &\multicolumn{1}{c}{57.3}   &\cellcolor{gray!30}52.5 && 71.6 & 65.7 &\multicolumn{1}{c}{40.6} & \cellcolor{gray!30}53.2& \cellcolor{gray!30}52.8\\
% \cmidrule{2-14}
% % \midrule
% & \multirow{2}{*}{\shortstack{Scene Debiasing}} & BE \cite{BE}  &   77.6&    44.3&    44.3& \multicolumn{1}{c}{52.0} &\cellcolor{gray!30}46.9& &&& 39.2 &\cellcolor{gray!30} &  \cellcolor{gray!30}\\
%  & & FAME \cite{fame} & 77.8 & 50.0  & 50.8  &  \multicolumn{1}{c}{57.0}  &\cellcolor{gray!30}52.6 && 70.3 & 64.9 &\multicolumn{1}{c}{36.8} &\cellcolor{gray!30}50.9 & \cellcolor{gray!30}51.6\\
% % \cline{1-14}

% \midrule

% Scene$\dagger$ & Naive & Baseline ViT & 43.0 & 9.8 & 8.0 & \multicolumn{1}{c}{15.8} & \cellcolor{gray!30}11.2 && 86.5&  82.6& \multicolumn{1}{c}{77.9} & \cellcolor{gray!30}80.3 & \cellcolor{gray!30}19.7 \\

% \midrule

%  & Multi-Task &  One-Token & 74.2 & 35.3 & 36.4 & \multicolumn{1}{c}{46.2} & \cellcolor{gray!30}39.3 & & 87.9 & \multicolumn{1}{c}{83.8} & 78.5 & \cellcolor{gray!30}81.2 & \cellcolor{gray!30}53.0 \\
% \cmidrule{2-14}
% % \midrule
% Action &  \multirow{4}{*}{Disentangle} & Two-Token & 75.1& 37.1   & 36.4     & \multicolumn{1}{c}{47.2} &\cellcolor{gray!30}40.2 && 86.4 & 75.8 & \multicolumn{1}{c}{81.5} &\cellcolor{gray!30}78.7&  \cellcolor{gray!30}53.2\\
%   \& & & Two-Token w/ BE \cite{BE} & 75.1 & 37.4 & 37.3 & 48.0& \cellcolor{gray!30}40.9 & & 87.7 & 82.9 & 75.9 &\cellcolor{gray!30}79.4 &\cellcolor{gray!30}54.0 \\
% Scene & & Two-Token w/ FAME \cite{fame} & 75.0 & 35.8  & 37.6    &\multicolumn{1}{c}{52.1} &\cellcolor{gray!30}41.8  && 87.3 & 77.4 &\multicolumn{1}{c}{82.7} & \cellcolor{gray!30}80.1& \cellcolor{gray!30}\second{54.9}\\
% % \cline{3-13}
%  & & DEVIAS & 77.3 & 51.8& 53.0&  \multicolumn{1}{c}{59.7} &\cellcolor{gray!30}54.8&& 82.0 &  76.5& \multicolumn{1}{c}{68.2} &\cellcolor{gray!30}72.3& \cellcolor{gray!30}\best{62.4}\\
%  % \midrule
% % \midrule
% % Scene & Naive & Baseline ViT & - & - & - & \multicolumn{1}{c}{-} & \cellcolor{gray!30}- && 72.0 & 61.7 & \multicolumn{1}{c}{41.5} & \cellcolor{gray!30}51.6 & \cellcolor{gray!30}- \\

% \bottomrule
% \end{tabular}

% }
% \label{tab:scuba}
% \end{table*}



% replace SCUBA-bg with HAT-bg
% \begin{table*}[t]
% \centering
% \caption{\textbf{Action and scene recognition performance on the Kinetics-400 dataset}. We report the Top-1 action recognition accuracy and the Top-5 scene recognition accuracy. We evaluate both in-context and out-of-context recognition performances. We also report the harmonic mean (H.M.) of the action recognition and scene recognition. The  \best{best} and the  \second{second-best} H.M. numbers are highlighted. $\dagger$ indicates evaluating the performance of contrasting supervision, we adapt linear probe.}

% \def\arraystretch{1.2}

% %\fontsize{7.5pt}{9.5pt}\selectfont
% \resizebox{1.0\linewidth}{!}{
% \begin{tabular}{ lll ccccc  c  ccccc c }
% \toprule

% \multirow{3}{*}{\shortstack{Supervision}} & \multirow{3}{*}{\shortstack{Training \\ Strategy}} &  \multirow{3}{*}{Method} & \multicolumn{5}{c}{Action($\uparrow$) } & \multicolumn{6}{c}{Scene($\uparrow$)} & \cellcolor{gray!30}\\
% \cline{4-8}
% \cline{10-14}
% & &  & In-Context & \multicolumn{4}{c}{SCUBA-Kinetics-400} && In-Context & \multicolumn{1}{c}{Kinetics-400} & \multicolumn{2}{c}{HAT-Kinetics-400}  &  &  \cellcolor{gray!30}H.M.\\
% \cline{5-8} \cline{11-14}
% & & & Kinetics-400 & Places365 & VQGAN-CLIP  & \multicolumn{1}{c}{Sinusoid} & \cellcolor{gray!30}Mean && Kinetics-400 &Scene-Only& Random & Far & \cellcolor{gray!30}Mean & \cellcolor{gray!30}\\

% \midrule
      
% \multirow{4}{*}{Action$\dagger$} & \multirow{2}{*}{Naive} &  Baseline ViT  &  76.8 & 42.3 &  43.5 &  \multicolumn{1}{c}{49.9} &\cellcolor{gray!30}45.2 &&   71.2&   65.8&  \multicolumn{1}{c}{63.3} & 65.7 & \cellcolor{gray!30}64.9 & \cellcolor{gray!30}53.3 \\
% & & \shortstack{Baseline ViT w/ Aug.} & 77.6 & 50.7&  49.4    &\multicolumn{1}{c}{57.3}   &\cellcolor{gray!30}52.5 && 71.6 & 65.7 &\multicolumn{1}{c}{63.9} & 65.7 & \cellcolor{gray!30}65.1& \cellcolor{gray!30}58.1\\
% \cmidrule{2-15}
% % \midrule
% & \multirow{2}{*}{\shortstack{Scene Debiasing}} & BE \cite{BE}  &   77.6&    44.3&    44.3& \multicolumn{1}{c}{52.0} &\cellcolor{gray!30}46.9& & 70.7 & 65.4 & 63.7 & 65.7 &\cellcolor{gray!30}64.9 &  \cellcolor{gray!30}54.5 \\
%  & & FAME \cite{fame} & 77.8 & 50.0  & 50.8  &  \multicolumn{1}{c}{57.0}  &\cellcolor{gray!30}52.6 && 70.3 & 64.9 &\multicolumn{1}{c}{61.7} & 64.5 &\cellcolor{gray!30}63.7 & \cellcolor{gray!30}\second{57.6}\\
% % \cline{1-14}

% \midrule

% Scene$\dagger$ & Naive & Baseline ViT & 43.0 & 9.8 & 8.0 & \multicolumn{1}{c}{15.8} & \cellcolor{gray!30}11.2 && 86.5&  82.6& \multicolumn{1}{c}{81.2} & 81.7 & \cellcolor{gray!30}81.8 & \cellcolor{gray!30}19.7 \\

% \midrule

%  & Multi-Task &  One-Token & 74.2 & 35.3 & 36.4 & \multicolumn{1}{c}{46.2} & \cellcolor{gray!30}39.3 & & 87.9 & \multicolumn{1}{c}{83.8} & 82.6 & 83.3 & \cellcolor{gray!30}83.2 & \cellcolor{gray!30}53.4 \\
% \cmidrule{2-15}
% % \midrule
% Action &  \multirow{4}{*}{Disentangle} & Two-Token & 75.1& 37.1   & 36.4     & \multicolumn{1}{c}{47.2} &\cellcolor{gray!30}40.2 && 86.4 & 75.8 & \multicolumn{1}{c}{80.1} & 81.4 &\cellcolor{gray!30}79.1&  \cellcolor{gray!30}53.3\\
%   \& & & Two-Token w/ BE \cite{BE} & 75.1 & 37.4 & 37.3 & 48.0& \cellcolor{gray!30}40.9 & & 87.7 & 82.9 & 81.4 & 83.1 &\cellcolor{gray!30}82.5 &\cellcolor{gray!30}54.7 \\
% Scene & & Two-Token w/ FAME \cite{fame} & 75.0 & 35.8  & 37.6    &\multicolumn{1}{c}{52.1} &\cellcolor{gray!30}41.8  && 87.3 & 77.4 &\multicolumn{1}{c}{81.9} & 84.0 & \cellcolor{gray!30}81.1& \cellcolor{gray!30}55.2\\
% % \cline{3-13}
%  & & DEVIAS & 77.3 & 51.8& 53.0&  \multicolumn{1}{c}{59.7} &\cellcolor{gray!30}54.8&& 82.0 &  76.5& \multicolumn{1}{c}{75.8} & 78.0 &\cellcolor{gray!30}76.8& \cellcolor{gray!30}\best{63.9}\\
%  % \midrule
% % \midrule
% % Scene & Naive & Baseline ViT & - & - & - & \multicolumn{1}{c}{-} & \cellcolor{gray!30}- && 72.0 & 61.7 & \multicolumn{1}{c}{41.5} & \cellcolor{gray!30}51.6 & \cellcolor{gray!30}- \\

% \bottomrule
% \end{tabular}

% }
% \label{tab:scuba}
% \end{table*}



% H.M. including in-context
% two H.M.
% \begin{table*}[t]
% \centering
% \caption{\textbf{Action and scene recognition performance on the Kinetics-400 dataset}. We report the Top-1 action recognition accuracy and the Top-5 scene recognition accuracy. We evaluate both in-context and out-of-context recognition performances. We also report the harmonic mean (H.M.) of the action recognition and scene recognition. The  \best{best} and the  \second{second-best} H.M. numbers are highlighted. $\dagger$ indicates that we are evaluating the performance under contrasting supervision, for which we employ a linear probe approach.}

% \def\arraystretch{1.2}

% %\fontsize{7.5pt}{9.5pt}\selectfont
% \resizebox{1.0\linewidth}{!}{
% \begin{tabular}{ lll ccccc  c  ccccc cc }
% \toprule

% \multirow{3}{*}{\shortstack{Supervision}} & \multirow{3}{*}{\shortstack{Training \\ Strategy}} &  \multirow{3}{*}{Method} & \multicolumn{5}{c}{Action($\uparrow$) } & \multicolumn{6}{c}{Scene($\uparrow$)} & \cellcolor{gray!30}w/o iid & \cellcolor{gray!30} w/ iid\\
% \cline{4-8}
% \cline{10-14}
% & &  & \multirow{2}{*}{\shortstack{In-Context}} & \multicolumn{4}{c}{Out-of-Context (SCUBA)} && \multirow{2}{*}{\shortstack{In-Context}} & \multicolumn{3}{c}{Out-of-Context (HAT)}  &  &  \cellcolor{gray!30}H.M. & \cellcolor{gray!30}H.M.\\
% \cline{5-8} \cline{11-14}
% & & & & Places365 & VQGAN-CLIP  & \multicolumn{1}{c}{Sinusoid} & \cellcolor{gray!30}Mean && &Scene-Only& Random & Far & \cellcolor{gray!30}Mean & \cellcolor{gray!30} & \cellcolor{gray!30}\\

% \midrule
      
% \multirow{4}{*}{Action$\dagger$} & \multirow{2}{*}{Naive} &  Baseline ViT  &  \cellcolor{gray!30}76.8 & 42.3 &  43.5 &  \multicolumn{1}{c}{49.9} &\cellcolor{gray!30}45.2 &&  \cellcolor{gray!30} 71.2&   65.8&  \multicolumn{1}{c}{63.3} & 65.7 & \cellcolor{gray!30}64.9 & \cellcolor{gray!30}53.3 & \cellcolor{gray!30}59.1\\
% & & \shortstack{Baseline ViT w/ Aug.} & \cellcolor{gray!30}77.6 & 50.7&  49.4    &\multicolumn{1}{c}{57.3}   &\cellcolor{gray!30}52.5 && \cellcolor{gray!30}71.6 & 65.7 &\multicolumn{1}{c}{63.9} & 65.7 & \cellcolor{gray!30}65.1& \cellcolor{gray!30}58.1 & \cellcolor{gray!30}\second{62.5}\\
% \cmidrule{2-16}
% % \midrule
% & \multirow{2}{*}{\shortstack{Scene Debiasing}} & BE \cite{BE}  &  \cellcolor{gray!30} 77.6&    44.3&    44.3& \multicolumn{1}{c}{52.0} &\cellcolor{gray!30}46.9& & \cellcolor{gray!30}70.7 & 65.4 & 63.7 & 65.7 &\cellcolor{gray!30}64.9 &  \cellcolor{gray!30}54.5 &\cellcolor{gray!30}59.9\\
%  & & FAME \cite{fame} & \cellcolor{gray!30}77.8 & 50.0  & 50.8  &  \multicolumn{1}{c}{57.0}  &\cellcolor{gray!30}52.6 && \cellcolor{gray!30} 70.3 & 64.9 &\multicolumn{1}{c}{61.7} & 64.5 &\cellcolor{gray!30}63.7 & \cellcolor{gray!30}\second{57.6} & \cellcolor{gray!30}62.0\\
% % \cline{1-14}

% \midrule

% Scene$\dagger$ & Naive & Baseline ViT & \cellcolor{gray!30}43.0 & 9.8 & 8.0 & \multicolumn{1}{c}{15.8} & \cellcolor{gray!30}11.2 && \cellcolor{gray!30}86.5&  82.6& \multicolumn{1}{c}{81.2} & 81.7 & \cellcolor{gray!30}81.8 & \cellcolor{gray!30}19.7 & \cellcolor{gray!30}31.1\\

% \midrule

%  & Multi-Task &  One-Token & \cellcolor{gray!30}74.2 & 35.3 & 36.4 & \multicolumn{1}{c}{46.2} & \cellcolor{gray!30}39.3 & & \cellcolor{gray!30}87.9 & \multicolumn{1}{c}{83.8} & 82.6 & 83.3 & \cellcolor{gray!30}83.2 & \cellcolor{gray!30}53.4 & \cellcolor{gray!30}61.2\\
% \cmidrule{2-16}
% % \midrule
% Action &  \multirow{4}{*}{Disentangle} & Two-Token & \cellcolor{gray!30}75.1& 37.1   & 36.4     & \multicolumn{1}{c}{47.2} &\cellcolor{gray!30}40.2 && \cellcolor{gray!30}86.4 & 75.8 & \multicolumn{1}{c}{80.1} & 81.4 &\cellcolor{gray!30}79.1&  \cellcolor{gray!30}53.3 & \cellcolor{gray!30}61.0\\
%   \& & & Two-Token w/ BE \cite{BE} & \cellcolor{gray!30}75.1 & 37.4 & 37.3 & 48.0& \cellcolor{gray!30}40.9 & & \cellcolor{gray!30}87.7 & 82.9 & 81.4 & 83.1 &\cellcolor{gray!30}82.5 &\cellcolor{gray!30}54.7 & \cellcolor{gray!30}62.2\\
% Scene & & Two-Token w/ FAME \cite{fame} & \cellcolor{gray!30}75.0 & 35.8  & 37.6    &\multicolumn{1}{c}{52.1} &\cellcolor{gray!30}41.8  && \cellcolor{gray!30}87.3 & 77.4 &\multicolumn{1}{c}{81.9} & 84.0 & \cellcolor{gray!30}81.1& \cellcolor{gray!30}55.2 & \cellcolor{gray!30}62.4\\
% % \cline{3-13}
%  & & DEVIAS & \cellcolor{gray!30}77.3 & 51.8& 53.0&  \multicolumn{1}{c}{59.7} &\cellcolor{gray!30}54.8&& \cellcolor{gray!30}82.0 &  76.5& \multicolumn{1}{c}{75.8} & 78.0 &\cellcolor{gray!30}76.8& \cellcolor{gray!30}\best{63.9} & \cellcolor{gray!30}\best{68.1}\\
%  % \midrule
% % \midrule
% % Scene & Naive & Baseline ViT & - & - & - & \multicolumn{1}{c}{-} & \cellcolor{gray!30}- && 72.0 & 61.7 & \multicolumn{1}{c}{41.5} & \cellcolor{gray!30}51.6 & \cellcolor{gray!30}- \\

% \bottomrule
% \end{tabular}

% }
% \label{tab:scuba_k400}
% \end{table*}




% \begin{table*}[t]
% \centering
% \caption{\textbf{Action and scene recognition performance on the Kinetics-400 dataset}. We report the Top-1 action recognition accuracy and the Top-5 scene recognition accuracy. We evaluate both in-context and out-of-context recognition performances. We also report the harmonic mean (H.M.) of the action recognition and scene recognition. The  \best{best} and the  \second{second-best} H.M. numbers are highlighted.}

% \def\arraystretch{1.2}

% %\fontsize{7.5pt}{9.5pt}\selectfont
% \resizebox{1.0\linewidth}{!}{
% \begin{tabular}{ l l l c  c c c c  cc  c c  c c }
% \toprule

% \multirow{3}{*}{\shortstack{Supervision}} & \multirow{3}{*}{\shortstack{Training \\ Strategy}} &  \multirow{3}{*}{Method} & \multicolumn{5}{c}{Action($\uparrow$) } & \multicolumn{5}{c}{Scene($\uparrow$)} & \cellcolor{gray!30}\\
% \cline{4-8}
% \cline{10-13}
% & &  & In-Context & \multicolumn{4}{c}{SCUBA-Kinetics-400} && In-Context & \multicolumn{1}{c}{Kinetics-400} & SCUBA-Kinetics-400  &  &  \cellcolor{gray!30}H.M.\\
% \cline{5-8} \cline{11-13}
% & & & Kinetics-400 & Places365 & VQGAN-CLIP  & \multicolumn{1}{c}{Sinusoid} & \cellcolor{gray!30}Mean && Kinetics-400 &Scene-Only& \multicolumn{1}{c}{Places365}  & \cellcolor{gray!30}Mean & \cellcolor{gray!30}\\

% \midrule
      
% \multirow{4}{*}{Action} & \multirow{2}{*}{Naive} &  Baseline ViT  &  92.9 & 15.0 &  12.4 &  \multicolumn{1}{c}{21.0} &\cellcolor{gray!30}16.1 && 62.9 & 50.2 &  \multicolumn{1}{c}{8.8} & \cellcolor{gray!30}29.5& \cellcolor{gray!30}20.8\\
% & & \shortstack{Baseline ViT w. Aug.} & 91.3& 19.1&  18.8    &\multicolumn{1}{c}{19.4}   &\cellcolor{gray!30}19.1 && 64.0 & 52.0 &\multicolumn{1}{c}{9.8} & \cellcolor{gray!30}30.9& \cellcolor{gray!30}23.6\\
% \cmidrule{2-14}
% % \midrule
% & \multirow{2}{*}{\shortstack{Scene Debiasing}} & BE \cite{BE}  & 92.3 & 16.1  & 12.1  & \multicolumn{1}{c}{38.7} &\cellcolor{gray!30}22.3 && 63.6 & 51.7 & \multicolumn{1}{c}{9.4} &\cellcolor{gray!30}30.5 &  \cellcolor{gray!30}25.8\\
%  & & FAME \cite{fame} & 91.6& 22.0  & 24.8  &  \multicolumn{1}{c}{15.6}  &\cellcolor{gray!30}20.8 && 62.7 & 51.2 &\multicolumn{1}{c}{9.3} &\cellcolor{gray!30}30.2 & \cellcolor{gray!30}24.6\\
% % \cline{1-14}

% \midrule

% Scene & Naive & Baseline ViT & - & - & - & \multicolumn{1}{c}{-} & \cellcolor{gray!30}- && 72.0 & 61.7 & \multicolumn{1}{c}{41.5} & \cellcolor{gray!30}51.6 & \cellcolor{gray!30}- \\

% \midrule

%  & Multi-Task &  One-Token & & 10.5 & 5.0 & \multicolumn{1}{c}{21.8} & \cellcolor{gray!30}12.4 & & & \multicolumn{1}{c}{60.5} & 20.9 & \cellcolor{gray!30}40.7 & \cellcolor{gray!30}19.0 \\
% \cmidrule{2-14}
% % \midrule
% Action &  \multirow{4}{*}{Disentangle} & Two-Token & 86.0& 11.9   &11.1     & \multicolumn{1}{c}{19.9} &\cellcolor{gray!30}14.3 && 72.3 & 59.6 & \multicolumn{1}{c}{18.4} &\cellcolor{gray!30}39.0&  \cellcolor{gray!30}24.6\\
%   \& & & Two-Token w. BE \cite{BE} & 89.9 &  15.0   &  13.0   & \multicolumn{1}{c}{20.5} &\cellcolor{gray!30}16.2 &&  74.2  & 62.3 & \multicolumn{1}{c}{19.4} & \cellcolor{gray!30}40.9 & \cellcolor{gray!30}23.2\\
% Scene & & Two-Token w. FAME \cite{fame} & 89.5 & 21.7  &25.3    &\multicolumn{1}{c}{15.3} &\cellcolor{gray!30}20.7  && 73.2 & 61.4 &\multicolumn{1}{c}{24.4} & \cellcolor{gray!30}42.9& \cellcolor{gray!30}\second{27.9}\\
% % \cline{3-13}
%  & & DEVIAS &90.1 & 41.0   &41.8    &  \multicolumn{1}{c}{40.6} &\cellcolor{gray!30}41.2 &&  73.3  &  60.2 & \multicolumn{1}{c}{20.9} &\cellcolor{gray!30}40.5 & \cellcolor{gray!30}\best{40.8}\\
%  % \midrule
% % \midrule
% % Scene & Naive & Baseline ViT & - & - & - & \multicolumn{1}{c}{-} & \cellcolor{gray!30}- && 72.0 & 61.7 & \multicolumn{1}{c}{41.5} & \cellcolor{gray!30}51.6 & \cellcolor{gray!30}- \\

% \bottomrule
% \end{tabular}
% }
% \label{tab:scuba}
% \end{table*}

==> table/rebuttal/cosine_ablation.tex <==
\vspace{-1em}
\begin{table}[h]
  \centering
  % \caption{\textbf{Ablation study on cosine similarity loss.} }
        \centering
        \resizebox{\linewidth}{!}{
        \begin{tabular}{lccccc}
            \toprule            
            \multirow{2}{*}{Method}& \multicolumn{2}{c}{UCF Action($\uparrow$)} & \multicolumn{2}{c}{UCF Scene($\uparrow$)} & \multirow{2}{*}{H.M.}\\
         \cmidrule(lr){2-3} \cmidrule(lr){4-5} 

        & In-Context & SCUBA-Places & In-Context & Scene-Only \\
            \midrule
         w/o cosine loss & 90.0 & 42.7 & 70.2 & 57.8 & 60.5 \\
         w/ cosine loss & 90.1 & 41.1  & 74.0 & 61.0 & \best{61.2} \\
           \bottomrule
        \end{tabular}
        }
\label{tab:cosine_abl}
\end{table}
\vspace{-1.5em}

==> table/rebuttal/downstream.tex <==
\begin{table}[h]
\centering
% \caption{\tb{Downstream task performance across multiple datasets.} We report top-1 accuracy. All models are pre-trained on the Kinetics-400 dataset. SSV2 denotes the Something-Something-V2 dataset.}
\resizebox{\linewidth}{!}{
\begin{tabular}{l cc c cc c}
    
\toprule
% \multirow{2}{*}{Supervision}&\multirow{2}{*}{Training Strategy}&\multirow{2}{*}{Method}&\multicolumn{2}{c}{Temporal-biased}&&\multicolumn{2}{c}{Static-biased} & \cellcolor{gray!30}\\
\multirow{2}{*}{Method}&\multicolumn{2}{c}{Temporal-biased}&&\multicolumn{2}{c}{Static-biased} & \\
\Xcline{2-3}{0.03em}
\Xcline{5-6}{0.03em}
 & Diving48 & SSV2&  & UCF-101 & SUN397&\multirow{-2}{*}{H.M.}\\
\midrule
% \multirow{2}{*}{Action}&\multirow{2}{*}{Naive}&Action ViT  & 81.5 &74.2&& 98.5 & 69.8 &\cellcolor{gray!30}79.6 \\
% &&Action ViT w/ Aug. &81.6 &74.5&& 98.5 & 68.4 & \cellcolor{gray!30}79.3\\
% \midrule
% \multirow{2}{*}{Action}&\multirow{2}{*}{Scene Debiasing}&BE~\cite{BE} & 81.9 &74.5&& 98.3 & 69.8 & \cellcolor{gray!30}79.8\\
% &&FAME~\cite{fame} & 80.6 &74.2& & 98.3 & 69.4& \cellcolor{gray!30}79.3\\
% \midrule
% \multirow{3}{*}{\begin{minipage}{0.5in}Action \& \\ Scene\end{minipage}}&\multirow{3}{*}{Disentangle}&Two-Token & 80.1 & 73.7&&98.2&73.5&\cellcolor{gray!30}80.3\\
Two-Token & 80.1 & 73.7&&98.2&73.5&80.3\\
% DEVIAS (sum.) & 81.6 & 74.6 && 98.0 & 71.4 & 80.2 \\
% DEVIAS (concat.) & 82.4 & 74.8 && 98.0 & 72.1 & 80.7 \\
% DEVIAS (concat.) & 82.9(+0.5) & 74.8 && 98.2(+0.2) & 72.1 & 80.7$\rightarrow$80.8 \\
DEVIAS (concat.) & 84.4 & 75.2 && 98.4 & 72.1 & 81.3\\
% DEVIAS (concat.)(14) & - & - && 98.8 & - & \cellcolor{gray!30}- \\

\bottomrule
\end{tabular}
}
\label{tab:downstream}
\end{table}

==> table/rebuttal/static_scene_model.tex <==
% \vspace{-1em}
\begin{table}[h]
  \centering
  % \caption{\textbf{Comparison with using additional static scene model.} }
        \centering
        \resizebox{\linewidth}{!}{
        \begin{tabular}{lccccc}
            \toprule            
            \multirow{2}{*}{Method}& \multicolumn{2}{c}{UCF Action($\uparrow$)} & \multicolumn{2}{c}{UCF Scene($\uparrow$)}  & \multirow{2}{*}{H.M.}\\
         \cmidrule(lr){2-3} \cmidrule(lr){4-5} 

        & In-Context & Out-of-Context & In-Context & Out-of-Context \\
            \midrule
             % Scene ViT& 69.2  & 3.4 & 72.0  & 64.7  & 11.8 \\
         % Static scene model (IN 1k mae) & - & - & 76.3 & 66.8  & - \\
         Static scene ViT  & 59.4 & 2.3 & 67.2 &  56.2 & 8.3 \\
         % Static scene model (ucf mae) & - & - &  &   & - \\
         % 65.1 70.2 65.1
         % Action ViT & 92.9 & 16.1 & 62.9 & 52.2 & 37.1  \\
         % Action ViT \& Static scene model (IN 1k mae) & 92.9 & 16.1 & 76.3 & 66.8  & 39.6 \\    
         % Action ViT \& scene ViT& 92.9 & 16.1 & 72.0  & 64.7 & 39.1 \\
         % Action ViT w/ BE \& scene ViT& 92.3 & 22.3& 72.0  & 64.7&47.0  \\
         % Action ViT w/ FAME \& scene ViT& 91.6 & 20.8& 72.0  & 64.7& 45.3 \\
         
         % Action ViT \& Static scene ViT& 92.9 & 16.1 & 67.2 &  56.2 &37.9  \\
         % Action ViT w/ BE \& Static scene ViT& 92.3 & 22.3&67.2 & 52.2& 44.6 \\
         FAME \& Static scene ViT& 91.6 & 20.8&67.2 & 52.2&43.0  \\
         DEVIAS & 90.1 & 40.0 & 74.0 & 64.5  & \best{61.4} \\
           \bottomrule
        \end{tabular}
        }
\label{tab:static_scene}
\end{table}
% \vspace{-1.5em}

==> table/supple/baseline_be.tex <==
\begin{table}[t]
\centering
\caption{\tb{Hyperparameters used for training the Two-Token w/ BE on each dataset.}}
\vspace{1em}

\resizebox{\columnwidth}{!}{
\begin{tabular}{lcc}
    
% \shline
\toprule
Config & UCF-101 & Kinetics-400 \\
% \shline
\midrule
Optimizer &   AdamW~\cite{adamw}& AdamW \\
Base learning rate &   5e-4 &1e-3 \\
Weight decay &   0.05 &0.05  \\
Optimizer momentum &   {$\beta_1, \beta_2 = 0.9, 0.999$}~\cite{chen2020generative}& {$\beta_1, \beta_2 = 0.9, 0.999$} \\
Per GPU batch size &    12&12 \\
Drop out & 0.5 & 0.0\\
Drop path& 0.2 & 0.1 \\
Color jitter&   0.4&0.4 \\
Flip augmentation & \checkmark & \checkmark \\
Mixup~\cite{zhang2017mixup} & $\times$ & $\times$ \\
Cutmix~\cite{yun2019cutmix} & $\times$ & $\times$ \\
Random erasing~\cite{zhong2020random} & $\times$ & $\times$\\
Mixing weight & $\sim \text{Uniform}(0,0.3)$ & $\sim \text{Uniform}(0,0.3)$\\
$\rho$ & 0.5 & 0.5 \\
Layer-wise learning rate decay~\cite{bao2021beit}&    0.75&0.75 \\
Learning rate schedule  & cosine decay~\cite{cosineannealing} & cosine decay\\
Warmup epochs & 5 & 5 \\
Training epochs &    100&100 \\
\bottomrule
\end{tabular}
}

\vspace{.2em}

\label{tab:baseline_be}
\end{table}



==> table/supple/baseline_fame.tex <==
\begin{table}[t]
\centering
\caption{\tb{Hyperparameters used for training the Two-Token w/ FAME on each dataset.}}
\vspace{1em}

\resizebox{\columnwidth}{!}{
\begin{tabular}{lcc}
    
% \shline
\toprule
Config & UCF-101 & Kinetics-400 \\
% \shline
\midrule
Optimizer &   AdamW~\cite{adamw}& AdamW \\
Base learning rate &   5e-4 &1e-3 \\
Weight decay &   0.05 &0.05  \\
Optimizer momentum &   {$\beta_1, \beta_2 = 0.9, 0.999$}~\cite{chen2020generative}& {$\beta_1, \beta_2 = 0.9, 0.999$} \\
Per GPU batch size &    12&12 \\
Drop out & 0.5 & 0.0\\
Drop path& 0.2 & 0.1 \\
Color jitter&   0.4&0.4 \\
Flip augmentation & \checkmark & \checkmark \\
Mixup~\cite{zhang2017mixup} & $\times$ & $\times$ \\
Cutmix~\cite{yun2019cutmix} & $\times$ & $\times$ \\
Random erasing~\cite{zhong2020random} & $\times$ & $\times$\\
$\tau$,$\rho$ & 0.5,0.5 & 0.5,0.5 \\
Layer-wise learning rate decay~\cite{bao2021beit}&    0.75&0.75 \\
Learning rate schedule  & cosine decay~\cite{cosineannealing} & cosine decay\\
Warmup epochs & 5 & 5 \\
Training epochs &    100&100 \\
\bottomrule
\end{tabular}
}

\vspace{.2em}

\label{tab:baseline_fame}
\end{table}



==> table/supple/baseline_noaug.tex <==
\begin{table}[t]
\centering
\caption{\tb{Hyperparameters used for training the disentangling baselines on each dataset.}}
\vspace{1em}
\resizebox{\columnwidth}{!}{
\begin{tabular}{lcc}
    
% \shline
\toprule
Config & UCF-101 & Kinetics-400 \\
% \shline
\midrule
Optimizer &   AdamW~\cite{adamw}& AdamW \\
Base learning rate &   5e-4 &5e-4 \\
Weight decay &   0.05 &0.05  \\
Optimizer momentum &   {$\beta_1, \beta_2 = 0.9, 0.999$}~\cite{chen2020generative}& {$\beta_1, \beta_2 = 0.9, 0.999$} \\
Per GPU batch size &    12&12 \\
Drop out & 0.5 & 0.0\\
Drop path& 0.2 & 0.1 \\
Color jitter&   0.4&0.4 \\
Flip augmentation & \checkmark & \checkmark \\
Mixup~\cite{zhang2017mixup} & $\times$ & $\times$ \\
Cutmix~\cite{yun2019cutmix} & $\times$ & $\times$ \\
Random erasing~\cite{zhong2020random} & $\times$ & $\times$\\
Layer-wise learning rate decay~\cite{bao2021beit}&    0.75&0.75 \\
Learning rate schedule  & cosine decay~\cite{cosineannealing} & cosine decay\\
Warmup epochs & 5 & 5 \\
Training epochs &    100&100 \\
\bottomrule
\end{tabular}
}
\vspace{.2em}

\label{tab:baseline_noaug}
\end{table}



==> table/supple/slot_assignment.tex <==
\begin{table}[h]
\centering

\caption{\textbf{Slot assignments in action recognition and scene recognition on UCF-101.}  We present the slot selection results of DEVIAS on UCF-101 dataset. We employ 4550 SCUBA-Places videos for action recognition and 3783 Scene-Only videos for scene recognition. The numbers inside the table mean the frequency of being selected for each column's slot.}

% \resizebox{0.9\columnwidth}{!}{
\fontsize{7.5pt}{9.5pt}\selectfont
\begin{tabular}{cc c c c c c}
\toprule
 && \multicolumn{2}{c}{Action} && \multicolumn{2}{c}{Scene} \\
\cline{3-4} \cline{6-7}
 && In-Context & Out-of-Context && In-Context & Out-of-Context \\
 && UCF-101 & SCUBA-Places && UCF-101 & Scene-Only \\

\midrule
\multirow{2}{*}{Slot 1} & Action Slot & - & 4550 && - & 3783 \\
 & Scene Slot & - & 0 && - & 0 \\

\midrule

\multirow{2}{*}{Slot 2} & Action Slot & - & 0 && - & 0 \\
 & Scene Slot & - & 4550 && - & 3783 \\

\bottomrule
\end{tabular}
\label{tab:slot_assign}
\end{table}

%%%%%%%%%%%%%%%%%%%%

\begin{table}[h]
\centering

\caption{\geo{Layout ?}}

% \resizebox{0.9\columnwidth}{!}{
\fontsize{7.5pt}{9.5pt}\selectfont
\begin{tabular}{ c | c | c | c }
\toprule
Dataset && Action Slot & Scene Slot \\

\midrule

\multirow{2}{*}{SCUBA-Places} & Slot 1 & 4550 & 0 \\
\cmidrule{2-4}
 & Slot 2 & 0 & 4550 \\

\midrule

\multirow{2}{*}{Scene-Only} & Slot 1 & 3783 & 0 \\
\cmidrule{2-4}
 & Slot 2 & 0 & 3783 \\

\bottomrule
\end{tabular}
\label{tab:slot_assign}
\end{table}

%%%%%%%%%%%%%%%%%%%%
\begin{table}[h]
\centering

\caption{\geo{Layout ?}}
    \mpage{0.48}{(a) Out-of-Context}
    \hfill
    \mpage{0.48}{(b) In-Context}
    \\
    \mpage{0.48}{
    % \resizebox{0.9\columnwidth}{!}{
    \fontsize{7.5pt}{9.5pt}\selectfont
    \begin{tabular}{c c  c  c  c }
    \toprule
    Dataset & Target && Action Slot & Scene Slot \\
    
    \midrule
    
    \multirow{2}{*}{SCUBA-Places} & \multirow{2}{*}{Action} & Slot 1 & 4550 & 0 \\
    \cmidrule{3-5}
     && Slot 2 & 0 & 4550 \\
    
    \midrule
    
    \multirow{2}{*}{Scene-Only} & \multirow{2}{*}{Scene} & Slot 1 & 3783 & 0 \\
    \cmidrule{3-5}
     && Slot 2 & 0 & 3783 \\
    
    \bottomrule
    \end{tabular}
    }
    \hfill
    \mpage{0.48}{
    % \resizebox{0.9\columnwidth}{!}{
    \fontsize{7.5pt}{9.5pt}\selectfont
    \begin{tabular}{c c  c  c  c }
    \toprule
    Dataset & Target && Action Slot & Scene Slot \\
    
    \midrule
    
    \multirow{4}{*}{UCF-101} & \multirow{2}{*}{Action} & Slot 1 & - & 0 \\
    \cmidrule{3-5}
     && Slot 2 & 0 & - \\
    
    \cmidrule{2-5}
    
     & \multirow{2}{*}{Scene} & Slot 1 & - & 0 \\
    \cmidrule{3-5}
     && Slot 2 & 0 & - \\
    
    \bottomrule
    \end{tabular}
    }
    
\label{tab:slot_assign}
\end{table}


    
%%%%%%%%%%%%%%%%%%%%
\begin{table}[h]
\centering

\caption{\geo{Layout ?}}

% \resizebox{0.9\columnwidth}{!}{
\fontsize{7.5pt}{9.5pt}\selectfont
\begin{tabular}{ c  c  c  c }
\toprule
Dataset && Action Slot & Scene Slot \\

\midrule

\multirow{2}{*}{SCUBA-Places} & Slot 1 & 4550 & 0 \\
 & \cellcolor{gray!30}Slot 2 & \cellcolor{gray!30}0 & \cellcolor{gray!30}4550 \\

\midrule

\multirow{2}{*}{Scene-Only} & Slot 1 & 3783 & 0 \\
 & \cellcolor{gray!30}Slot 2 & \cellcolor{gray!30}0 & \cellcolor{gray!30}3783 \\

\bottomrule
\end{tabular}
\label{tab:slot_assign}
\end{table}


==> table/ucf101_extra.tex <==
\begin{table*}[t]
\centering
\caption{\textbf{Action and scene recognition performance on the UCF-101 dataset}. We report the Top-1 action recognition accuracy and the Top-5 scene recognition accuracy. We evaluate both in-context and out-of-context recognition performances. We also report the harmonic mean (H.M.) of the action recognition and scene recognition. The  \best{best} and the  \second{second-best} H.M. numbers are highlighted. $\dagger$ indicates that we are evaluating the performance under contrasting supervision, for which we employ a linear probe approach.}

\def\arraystretch{1.2}

%\fontsize{7.5pt}{9.5pt}\selectfont
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{ lll c ccc ccc c  c  c c ccc c c }
\toprule

\multirow{3}{*}{\shortstack{Supervision}} & \multirow{3}{*}{\shortstack{Training \\ Strategy}} &  \multirow{3}{*}{Method} & \multicolumn{8}{c}{Action($\uparrow$) } & \multicolumn{7}{c}{Scene($\uparrow$)} & \cellcolor{gray!30}w/o iid \\
\cline{4-11}
\cline{13-18}
& &  & \multirow{2}{*}{In-Context} & \multicolumn{3}{c}{SCUBA} & \multicolumn{3}{c}{HAT} &&& \multirow{2}{*}{In-Context} & \multicolumn{4}{c}{HAT}  &  & \cellcolor{gray!30}H.M.\\
\cline{5-11} \cline{14-18}
& & &  & Places365 & VQGAN-CLIP  & Sinusoid & Random & Close & \multicolumn{1}{c}{Far} & \cellcolor{gray!30}Mean &&  &Scene-Only& Random & Close & Far & \cellcolor{gray!30}Mean & \cellcolor{gray!30}\\

\midrule
      
\multirow{4}{*}{Action$\dagger$} & \multirow{2}{*}{Naive} &  Baseline ViT  &  92.9 & 15.0 & 12.4 & 21.0 & & & &\cellcolor{gray!30}&&   62.9&   50.2 &  49.8 & 50.6 & 55.9  & \cellcolor{gray!30}& \cellcolor{gray!30}\\
& & \shortstack{Baseline ViT w/ Aug.} & 90.0 & 19.1 & 18.8 & 19.4 & & & &\cellcolor{gray!30}&& 64.0 & 52.0 & 52.6 & 50.4 & 62.0   &  \cellcolor{gray!30}& \cellcolor{gray!30}\\
\cmidrule{2-19}
% \midrule
& \multirow{2}{*}{\shortstack{Scene Debiasing}} & BE \cite{BE}  & 92.3 & 16.1 & 12.1 & 38.7 & & & &\cellcolor{gray!30}& & 63.6 & 51.7 & 52.4 & 52.4 &58.5 &\cellcolor{gray!30}&  \cellcolor{gray!30}\\
 & & FAME \cite{fame} & 91.6 & 22.0 & 24.8 & 15.6 & & & &\cellcolor{gray!30}&& 62.7 & 51.2 & 48.3 & 50.5 & 54.0 &\cellcolor{gray!30}& \cellcolor{gray!30}\second{}\\
% \cline{1-14}

\midrule

Scene$\dagger$ & Naive & Baseline ViT & 69.2 & 2.2 & 0.9 & 7.1 & & & & \cellcolor{gray!30}&& 72.0 & 61.7 & 62.3 & 60.6 & 69.3 & \cellcolor{gray!30}& \cellcolor{gray!30} \\

\midrule

 & Multi-Task &  One-Token & 91.9 & 10.5 & 5.0 & 21.8 & & & & \cellcolor{gray!30}& & 74.0 & 60.5 & 57.3 & 58.0 & 67.3 & \cellcolor{gray!30} & \cellcolor{gray!30} \\
\cmidrule{2-19}
% \midrule
Action &  \multirow{4}{*}{Disentangle} & Two-Token & 86.0 & 11.9 & 11.1 & 19.9 & & & &\cellcolor{gray!30}&& 72.3 & 59.6 & 59.2 & 57.9 & 66.9 &\cellcolor{gray!30}&  \cellcolor{gray!30}\\
  \& & & Two-Token w/ BE \cite{BE} & 89.9 & 15.0 & 13.0 & 20.5 & & & & \cellcolor{gray!30}& & 74.2 & 62.3 & 59.3 & 59.0 & 69.1 &\cellcolor{gray!30} &\cellcolor{gray!30} \\
Scene & & Two-Token w/ FAME \cite{fame} & 895 & 21.7 & 25.3 & 15.3 & & & & \cellcolor{gray!30}&& 73.2 & 61.4 & 63.2 & 60.9 & 70.4 & \cellcolor{gray!30}& \cellcolor{gray!30}\\
% \cline{3-13}
 & & DEVIAS & 90.1 & 41.0 & 41.8 & 40.6 & & & &\cellcolor{gray!30}&& 73.3 & 60.2 & 61.2 & 60.8 & 70.6 &\cellcolor{gray!30}& \cellcolor{gray!30}\best{}\\
 % \midrule
% \midrule
% Scene & Naive & Baseline ViT & - & - & - & \multicolumn{1}{c}{-} & \cellcolor{gray!30}- && 72.0 & 61.7 & \multicolumn{1}{c}{41.5} & \cellcolor{gray!30}51.6 & \cellcolor{gray!30}- \\

\bottomrule
\end{tabular}

}
\label{tab:scuba}
\end{table*}
